Community detection over a heterogeneous population of non-aligned networks

Clustering and community detection with multiple graphs have typically focused on aligned graphs, where there is a mapping between nodes across the graphs (e.g., multi-view, multi-layer, temporal graphs). However, there are numerous application areas with multiple graphs that are only partially aligned, or even unaligned. These graphs are often drawn from the same population, with communities of potentially different sizes that exhibit similar structure. In this paper, we develop a joint stochastic blockmodel (Joint SBM) to estimate shared communities across sets of heterogeneous non-aligned graphs. We derive an efficient spectral clustering approach to learn the parameters of the joint SBM. We evaluate the model on both synthetic and real-world datasets and show that the joint model is able to exploit cross-graph information to better estimate the communities compared to learning separate SBMs on each individual graph.

==> consistency_.tex <==
%


%
\subsection{Consistency}
\label{sec:consist}
%
The global parameter $\bm{\Theta}$ is central in order to understand Multi-graph settings. It not only gives an overall summary of how nodes connect based on their communities, but $\bm{\Theta}$ also has the role to link all graphs. In other words, a reliable estimate of $\bm{\Theta}$ means we can predict edges between nodes in different graphs with confidence. Here, we discuss the asymptotic behavior of $\bm{\Theta}$ in Multi-graph joint SBM as $N\rightarrow \infty$. And, we show that the estimator $\widehat{\bm{\Theta}}=N^{-1}\sum_n\widehat{\bm{\Theta}}_n$ in Eq.~\eqref{eq:theta_estimator_n} converge to the global $\bm{\Theta}$ almost surely for when we know the true membership. Lemma \ref{lemma:consistency_theta} (below) formalizes these statements. 

\begin{lemma}
Let the pair $(\bm{X},\bm{\Theta})$ parametrize a SBM with $K$ communities for $N$ graphs where $\bm{X}$ contains the membership matrix of all graphs stacked and $\bm{\Theta}$ is full rank. Write $\nu \le \min_n |V_n|$. Now if assume $(\widehat{\bm{W}},\widehat{\bm{X}})$ is the optimal solution of Eq.~\ref{eq:opt_kmeans_graphLevel} then $\widehat{\bm{\Theta}}$ converge to $\bm{\Theta}$ in probability Eq.~\eqref{eq:theta_weak_consistent}. If we also assume $\widehat{\bm{X}}_n = \bm{X}_n$ then $\widehat{\bm{\Theta}}$ converge to $\bm{\Theta}$ almost surely Eq.~\eqref{eq:theta_consistent}.
\vspace{-8mm}
\begin{multicols}{2}
\begin{equation}
\lim_{\nu\rightarrow \infty;N\rightarrow \infty} \widehat{\bm{\Theta}} \stackrel{P}{\rightarrow }\bm{\Theta}
\label{eq:theta_weak_consistent} 
 \end{equation}
\begin{equation}
\lim_{N\rightarrow \infty} \widehat{\bm{\Theta}} \stackrel{a.s.}{\rightarrow }\bm{\Theta}
\label{eq:theta_consistent} 
 \end{equation}
\end{multicols}
\label{lemma:consistency_theta}
\end{lemma}
%
%
%
%
%
%
%
%
%

\begin{comment} %
\begin{lemma}
Let the pair $(\bm{X},\bm{\Theta})$ parametrize a SBM with $K$ communities for $N$ graphs where $\bm{X}$ contains the membership matrix of all graphs stacked and $\bm{\Theta}$ is full rank. Also, let $\bm{X}_{ni}\stackrel{ind}{\sim}\text{Mult}(\bm{\pi}_n)$ where $\|\bm{\pi}_n\|_0 = K$, i.e. each graph has a positive probability to contain any of the $K$ communities.
Write also $\bm{U}_n\bm{D}_n\bm{U}_n^{T}$ and $\widehat{\bm{U}}_n\widehat{\bm{D}}_n\widehat{\bm{U}}_n^{T}$ as the eigendecomposition of $\bm{P}_n$ and $\bm{A}_n$ where  $\mathbb{E}[\bm{A}_n] = \bm{P}_n - diag(\bm{P}_n)$.
Now assume $(\widehat{\bm{W}},\widehat{\bm{X}})$ is a close enough approximate solution of Eq.~\ref{eq:kmeans_final} (e.g. $\mathcal{O}(\log{K})$-approximate using kmeans++ initialization in Algorithm \ref{algo:jointSpec2}). Define the number of misclustered nodes as $|S|:=\|\widehat{\bm{X}} - \bm{X}\|_0/2$. Finally, we have:
\vspace{-8mm}
\begin{multicols}{2}
  \begin{equation}
\lim_{N\rightarrow \infty} \frac{|S|}{|V|} \stackrel{P}{\rightarrow} 0
\label{eq:misclus_consistent} 
  \end{equation}
\begin{equation}
\lim_{N\rightarrow \infty} \widehat{\bm{\Theta}} \rightarrow \bm{\Theta}
\label{eq:theta_consistent} 
  \end{equation}
\end{multicols}
\label{lemma:consistency}
\end{lemma}
\end{comment}
%
\vspace{-4mm}
\textit{\textbf{Proof}} Eq.\eqref{eq:theta_weak_consistent} follows directly from the fact that $\bm{A}_n$ converge in probability to $\bm{P}_n$ for large $|V_n|$, Theorem 5.2~\cite{lei2015consistency}. Eq.\eqref{eq:theta_consistent} follows from Eq.~\eqref{eq:expected_estimator_n}, we know that $\mathbb{E}[\widehat{\bm{\Theta}}_n] = \bm{\Theta}$. 
%
Thus, using Kolmogorov-Khintchine strong law of large numbers,  $\widehat{\bm{\Theta}} \rightarrow \bm{\Theta}$ almost surely for large $N$. 

\vspace{-2mm}
$\hfill \qquad \qquad \qquad \qquad \qed$

%
%

Eq.~\eqref{eq:theta_consistent} is only true in the Multi-graph joint case. In the Isolated setting, we need to \textit{re-align} the memberships across graphs which adds an extra layer of complexity. For instance, assume the re-alignment procedure consists on (1) rank each community on each graph based on  $diag(\bm{\Theta}_n)$, then (2) re-order the connectivity matrix and membership accordingly. In this case, $Var(\widehat{\bm{\Theta}}) = \sum_n^N Var(\bm{\Theta}_n) \rightarrow \infty$, unless we assume graph size to be large, i.e. $\nu\rightarrow \infty$ where $ \nu \le \min_n|V_n|$. Nevertheless, this gives weak consistency at most. In fact, this is true for any realignment procedure whose performance is a function of graph size. Figure \ref{fig:syn_theta_dist} in the Synthetic experiments shows that the Joint model estimates $\bm{\Theta}$ well even for small graph settings which is not true for Isolated models. 

%
%
%

%


%


%

%
%

%
%
%

%

%

%

%
%
 %
%
%
%
%
%
%
%
%
%
%


\begin{comment}
\subsubsection{Goodness-of-fit}

The main assumption of the homogeneous scenario is that the number of nodes per graph in each cluster follows the same distribution, in other words $\bm{{m}}_n := |G_{n1}|,\dots,|G_{nK}| \stackrel{iid}{\sim} \text{Mult}(\bm{\zeta})$ for all $n$. Thus, if all graphs follow the same distribution of nodes over clusters, then $\bm{{M}} := |G_{\cdot1}|,\dots,|G_{\cdot K}| \stackrel{iid}{\sim} \text{Mult}(\bm{\zeta})$. Thus, we consider the following hypothesis testing for each graph
\begin{equation}
\begin{aligned}
  \mathcal{H}_0^{n}:& \ \bm{{m}}_n, \bm{{M}}^{-n} \stackrel{iid}{\sim} \text{Mult}(\bm{\zeta}),  \\
              & \ \bm{\zeta} \sim \text{Dirichlet}(\bm{\alpha}) \\
  \mathcal{H}_1^{n}:& \ \bm{{m}}_n \sim \text{Mult}(\bm{\zeta}_1) \ \ \text{and} \ \ \bm{{M}}^{-n} \sim \text{Mult}(\bm{\zeta}_2) \\
              & \ \bm{\zeta_1},\bm{\zeta_2} \sim \text{Dirichlet}(\bm{\alpha}) 
\end{aligned}
\label{overall_hyp}
\end{equation}

where $\bm{{M}}^{-n}:=|G_{\cdot1}| - |G_{n1}|,\dots,|G_{\cdot K}| - |G_{n K}|$. We can specify the posterior as
$$P(\mathcal{H}_1^{n}|-) = \frac{P(\bm{{m}}_n|\bm{\alpha})P(\bm{{M}}^{-n}|\bm{\alpha})}{P(\bm{{M}}|\bm{\alpha})+P(\bm{{m}}_n|\bm{\alpha})P(\bm{{M}}^{-n}|\bm{\alpha})}$$

Using the Dirichlet-multinomial conjugacy, the marginal probability of the alternative hypothesis is given by

\begin{equation}
P(\mathcal{H}_1^{n}|-) = \frac{\frac{B(\bm{\alpha}+\bm{{m}}_n)}{B(\bm{\alpha})}\frac{B\left(\bm{\alpha}+\bm{M}^{-n}\right)}{B(\bm{\alpha})} }{\frac{B(\bm{\alpha}+ \bm{{M}})}{B(\bm{\alpha})}+ \frac{B(\bm{\alpha}+\bm{{m}}_n)}{B(\bm{\alpha})}\frac{B\left(\bm{\alpha}+\bm{M}^{-n}\right)}{B(\bm{\alpha})} }
\label{probab}
\end{equation}
where $B(\cdot)$ is the multivariate beta function $B(x) = \prod_{i=1}^q\frac{\Gamma(x_i)}{\Gamma(\sum_{i=1}^q x_i)}$.  For more details, see \cite{durante2016,gomes2018multiple}. Thus, we have $P(\mathcal{H}_1^{n}|-)$ for each graph. For a given threshold $\varepsilon$, say $\varepsilon = .05$, our goodness-of-fit measure is given by 

\begin{equation}
\phi(\bm{X}|\varepsilon) = N^{-1} \sum_n \mathds{I}_{P(\mathcal{H}_1^{n}|-)>1-\varepsilon}
\end{equation} 

Overall, $\phi(\bm{X}|\varepsilon)$ gives the proportion of the graphs considered heterogeneous. Thus, for $\phi(\bm{X}|\varepsilon) \approx 0$ we should set $\gamma_n(\bm{X})=1$, otherwise we should perform Algorithm \ref{algo:jointSpec} as is.
\end{comment}
 %
 %

%
%
%


%
%
%
%
%
%
%
%
%
%
%
%
\begin{comment}
%
We have defined $f(\bm{\nu}) = \bm{\nu}\bo{Z}_n'\Delta_n^{-1}\Delta\bo{Z}$ and \gui{$\bm{\mu}(\bm{\nu}_i)=\frac{\sum_i\nu_i}{|\nu|}$}, $\bo{W}_{k}$ is the $k$-th row of $\bo{W}$ and $\bo{q}_{ni}$ is the $i$-th row of matrix $\bo{Q}_n$, thus $\bm{\mu}\left(f(\bm{q}_{ni})\right)=\bo{W}_k$.

Note that we do not observe $\bo{Z}_n$ or $\bo{Z}$ and those terms cannot be estimated trivially. Therefore, we aim to find a upper bound for Equation \eqref{eq:k_mean_global_openedterms} that does not depend on $f(\cdot)$. 
%
%
%
Using Taylor series expansion centered at $\bm{\mu}\left(\bo{q}_{ni}\right)$, we have
$$
\begin{aligned}
 f(\bm{q}_{ni}) &\approx f(\bm{\mu}\left(\bm{q}_{ni}\right) + \left[\left(\bo{q}_{ni} - \bm{\mu}\left(\bm{q}_{ni}\right) \right) \cdot \nabla f\left(\bm{\mu}[\bm{q}_{ni}]\right) \right]  \\
 \end{aligned}
$$
Thus, 
$$
\begin{aligned}
\sum_{k=1}^K \sum_{n=1}^N \sum_{i \in G_{nk}}  \|\bm{\mu}\left(f(\bo{q}_{ni})\right) - f(\bm{q}_{ni})\|^2 &= \sum_{k=1}^K \sum_{n=1}^N \sum_{i \in G_{nk}}  \|\bm{\mu}\left(f(\bo{q_{ni}})\right) - f\left(\bm{\mu}\left(\bm{q}_{ni}\right)\right) -  \left[\left(\bo{q}_{ni} - \bm{\mu}\left(\bm{q}_{ni}\right) \right) \cdot \nabla f\left(\bm{\mu}\left(\bm{q}_{ni}\right)\right) \right]\|^2 \\
&= \gui{\text{Based on Jensen's inequality, } f(\mu(\cdot)) = \mu(f(\cdot)) \text{ given } f(\cdot) \text{is linear}}\\
&=\gui{\sum_{k=1}^K \sum_{n=1}^N \sum_{i \in G_{nk}}  \| \bo{W}_k -  \bo{W}_k -  \left[\left(\bo{q}_{ni} - \bm{\mu}\left(\bm{q}_{ni}\right) \right) \cdot \nabla f\left(\bm{\mu}\left(\bm{q}_{ni}\right)\right) \right]\|^2} \\
 &= \sum_{k=1}^K \sum_{n=1}^N \sum_{i \in G_{nk}}  \|\left(\bo{q}_{ni} - \bm{\mu}\left(\bm{q}_{ni}\right)\right) \cdot \bo{Z}_n'\Delta_n^{-1}\Delta\bo{Z}  \|^2 \\
 &\le \sum_{k=1}^K \sum_{n=1}^N \sum_{i \in G_{nk}}  \|\bo{q}_{ni} - \bm{\mu}\left(\bm{q}_{ni}\right) \|^2 \| \bo{Z}_n'\Delta_n^{-1}\Delta\bo{Z}  \|\\
 &= \sum_{k=1}^K \sum_{n=1}^N \sum_{i \in G_{nk}}  \|\bo{q}_{ni} - \bm{\mu}\left(\bm{q}_{ni}\right) \|^2 \underbrace{\left( \max_m{\sqrt{\frac{|G_{\cdot m}|}{|G_{nm}|}}} \right)}_{\gamma_n} \\
 \end{aligned}
 $$
%
In summary, our overall optimization problem is given by
\begin{equation}
\begin{aligned}
(\widehat{\bo{W}},\widehat{\bm{X}}) &=
 \arg \min_{G_{\cdot \cdot},\bm{W} \in \mathbb{R}^{K \times K}}
\sum_{n=1}^N  \sum_{k=1}^K  \sum_{i \in G_{nk}} \left\|\widehat{\bo{q}}_{ni} - \bm{\mu}\left(\widehat{\bo{q}}_{ni}\right) \right\|^2 \gamma_n  \\
\end{aligned}
\label{eq:k_mean_global_per_graph}
\end{equation}
We optimize this using the usual Lloyd heuristic from the k-means 
algorithm. This involves iterating two simple steps: (1) compute centers 
of mass given observations in each cluster; (2) assign observations to 
clusters based on the closest center. 
%
%
%
We outline this process as follows:  
\begin{enumerate}
  \item For each community compute the location for the global center as
  $$
\begin{aligned}
  \bo{W} &= \Delta^{-2}\stacked{X}'\stacked{\bo{Q}}
\end{aligned} 
  $$
  \item For each graph 
  %
    %
    Estimate $\widehat{\gamma}_n = \max_m \sqrt{\frac{|G_{\cdot m}|}{|G_{nm}|}}$
    %
    %
  %
  \item For each node on each graph
  \begin{enumerate}
    \item Compute the square distance from each center as
    \begin{equation}
    \lambda_{nik} = \| \widehat{\bo{q}}_{ni} - \bo{W}_{k} \|^2 \widehat{\gamma}_n
    \label{eq:comp_dist}
    \end{equation}
    \item Assign node $i$ of graph $n$ to the cluster $\widehat{k} = \arg \min_k \lambda_{nik}$
  \end{enumerate}
\end{enumerate}
\end{comment}
%
%
%
%
%

%

%

%
%
%
%
%

%
%
%
%
%
%
%
%
%
%

%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
 %
 %
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%



==> fig1_algo1.tex <==
% \vspace{9mm}
% \begin{wrapfigure}{R}{0.5\textwidth}
\begin{minipage}{0.47\textwidth}
\begin{figure}[H]
    \centering
    \includegraphics[height=4.5in]{figures/synthetic_theta_distribution_transposed.pdf}
	\caption{Distribution of blocks for $5$, $50$, $100$, $200$ graphs (top) and synthetic data: True connectivity matrix $\bm{\Theta}$ (bottom).}
	\label{fig:syn_theta_dist}
\end{figure}
\end{minipage}
\begin{minipage}{0.47\textwidth}
\begin{algorithm}[H]
\caption{JointSpec SBM}\label{algo:jointSpec2}
 \begin{algorithmic}
 \STATE \textbf{Input}  $N$ adjacency matrices $\bm{A}_n  \in \{0,1\}^{|V_n| \times |V_n|}$, number of communities $K$ and tolerance  $\varepsilon$
 \FOR{$n \in [1,...,N]$}
 \STATE \textbf{Compute} $\widehat{\bo{U}}_n \in \mathbb{R}^{|V_n| \times K} $ and $\widehat{\bo{D}}_n \in \mathbb{R}^{K \times K}$ as the leading $K$  eigenvectors and eigenvalues of $\bo{A}_n $. \\
\STATE \textbf{set} $\widehat{\bo{Q}}^*_n \gets |\widehat{\bo{U}}_n\widehat{\bo{D}}_n|\sqrt{\frac{|V|}{|V_n|}}$
\STATE \textbf{Initialize} 
$\widehat{\bm{X}}_n$ randomly\\
\STATE \textbf{set}  $\widehat{\Delta}_n^2 \gets \widehat{\bm{X}}_n^T\widehat{\bm{X}}_n$ \\
\ENDFOR
\STATE \textbf{compute}  $\widehat{\Delta}^2 \gets \sum_n^N \widehat{\Delta}_n^2$ \\
\STATE \textbf{set}  $\text{loss}_0 \gets 0$,  $\text{loss}_1 \gets 1$ and $t \gets 1$ \\
 \WHILE{$|\text{loss}_{t} - \text{loss}_{t-1}| > \varepsilon$}
 \STATE \textbf{update}  $t \gets t + 1$ \\
 \FOR{$n \in [1,...,N]$}
 \STATE \textbf{compute}  $\gamma_n \gets \text{tr}(\widehat{\Delta}_n^2\widehat{\Delta}^{-2}) $ \COMMENT{Eq. \eqref{eq:def_gamman}}
\ENDFOR
 % \State $\Delta \gets \left[\bo{X}'\bo{X}\right]^{1/2}$
 % \State \textbf{update} $\widehat{\bo{W}}_n \gets \left[\bo{X}_n^{T}\bo{X}_n\right]^{-1}\bo{X}_n^{T}\widehat{\bo{Q}}_n$ 
 % \Comment{given by eq. \eqref{eq:local_mean}}
 \STATE \textbf{update} $\widehat{\bo{W}}$ \COMMENT{Eq. \eqref{eq:w_update_rule}}
 % \Comment{given by eq. \eqref{eq:global_mean}}
 \FOR{$n \in [1,...,N]$}
% \STATE \textbf{update}  $\gamma_n \gets tr(\widehat{\Delta}_n^2\widehat{\Delta}^{-2}) $ \COMMENT{given by eq. \eqref{eq:def_gamman}}
  \FOR{$i \in [1,...,|V_n|]$}
    \FOR{$k \in [1,...,K]$}
      \STATE \textbf{compute} $\tilde{\Delta}_{ni}(k)$ \COMMENT{Eq. \eqref{eq:def_gammaTilde}}
       \STATE \textbf{compute} $\omega_{ni}(k)$ \COMMENT{Eq. \eqref{eq:def_omega2}}
    \ENDFOR
    \STATE \textbf{update} $\widehat{\bo{X}}_{ni} \gets \text{onehot} (\argmin_k \omega_{ni}(k))$
    \ENDFOR
    \STATE \textbf{compute}  $\widehat{\Delta}_n^2 \gets \widehat{\bm{X}}_n^T\widehat{\bm{X}}_n$ \\
    \STATE \textbf{update}  $\eta_n(\widehat{\bm{X}}_n,\widehat{\bm{W}})$ \COMMENT{Eq. \eqref{eq:opt_kmeans_graphLevel_v3}} \\
\ENDFOR
 \STATE \textbf{compute}  $\widehat{\Delta}^2 \gets \sum_n^N \widehat{\Delta}_n^2$ \\
 \STATE \textbf{compute}  $\text{loss}_t\gets \sum_n^N \eta_n(\widehat{\bm{X}}_n,\widehat{\bm{W}})$
 \ENDWHILE
 % \State \textbf{Output} $\widehat{\bo{X}},\widehat{\widetilde{\bo{W}}}$
 \end{algorithmic}
\end{algorithm} 
\end{minipage}
%  \end{wrapfigure}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

